PAV: Personalized Head Avatar from Unstructured Video Collection

We propose PAV, Personalized Head Avatar for the synthesis of human faces under arbitrary viewpoints and facial expressions. PAV introduces a method that learns a dynamic deformable neural radiance field (NeRF), in particular from a collection of monocular talking face videos of the same character under various appearance and shape changes. Unlike existing head NeRF methods that are limited to modeling such input videos on a per-appearance basis, our method allows for learning multi-appearance NeRFs, introducing appearance embedding for each input video via learnable latent neural features attached to the underlying geometry. Furthermore, the proposed appearance-conditioned density formulation facilitates the shape variation of the character, such as facial hair and soft tissues, in the radiance field prediction. To the best of our knowledge, our approach is the first dynamic deformable NeRF framework to model appearance and shape variations in a single unified network for multi-appearances of the same subject. We demonstrate experimentally that PAV outperforms the baseline method in terms of visual rendering quality in our quantitative and qualitative studies on various subjects.

==> figures/fig_dataset.tex <==
\begin{table}[h]
    \centering
    % \small
    \setlength{\tabcolsep}{2mm}{
    \vspace{2pt}
    \renewcommand\arraystretch{0.99}
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{ccc} 
    \toprule
    \toprule
    \bf Subject & \bf {Number of} & \bf {Frames} \\ 
    & \bf {Appearances} & \bf {}   \\ 
    \midrule
    \midrule
    \bf Roger Federer & 5 & \{800,300,400,600,800\} \\
    \bf King Charles & 5 & \{800,300,400,600,800\}  \\
    \midrule
    \bottomrule
    \end{tabular}}}
    \caption{Video Collection Dataset} 
    \label{tab:dataset}
\end{table}

==> figures/fig_teaser.tex <==

\twocolumn[
{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \captionsetup{type=figure}
    \includegraphics[width=0.8\textwidth]{figures/teaser/teaser_v3.png}
    %\caption{We present, PAV, an approach for learning personalized head avatars from the unstructured collection of videos. Training frames from diverse set of appearances of the character are shown on the left. PAV can synthesize images of the person under target appearances, novel head poses, and facial expressions. On the right-hand side of the figure, we show a few samples observed in the training set (red frames) and our renderings for unseen appearances, poses, and expressions.}
    \caption{We present an approach for learning personalized head avatars from an unstructured video collection. %using a single unified dynamic deformable NeRF framework.
    The videos are taken in different environments, with diverse appearances and possible shape changes of a character, as shown on the left.
    Our method leverages all of the input clips into a single unified dynamic deformable NeRF framework and offers high-quality video replays in novel head pose and facial expression.
    On the right, we show some rendering results of each input aligned in head pose and facial expression.
    }
    \label{fig:teaser}
\end{center}%
}
]


==> sec/0_abstract_backup.tex <==
\begin{abstract}
% \bk{a}
% \ac{b}
% \hk{c}

% We propose PAV, a new approach for generating human avatars capable of adopting diverse facial expressions, appearances, and viewpoints. PAV leverages a novel technique that utilizes a dynamic, deformable neural radiance field (NeRF) model. This model is trained using a series of monocular videos of the same individual undergoing various changes in appearance while speaking.


%This methodology ensures a highly adaptable and realistic synthesis of human heads. NeRFs for dynamic head synthesis have shown 

We propose PAV, a personalized head avatar for the synthesis of humans under arbitrary viewpoints, facial expressions, and appearances. PAV introduces a method that learns a dynamic deformable neural radiance field (NeRF) from the collection of monocular in-the-wild talking face videos of same the character under various appearance changes. Although dynamic head NeRF methods have shown remarkable results in modeling and controlling faces; however, they require per-appearance optimization. To address this, to the best of our knowledge, we present the first single unified network that models complex head poses and facial expressions for multiple appearances of the same subject. The core contribution of our paper is that PAV proposes appearance embedding using learnable latent neural features attached to the underlying geometry and introduces appearance-conditioned density and radiance field prediction to learn multi-appearance face synthesis. In quantitative and qualitative studies on various subjects, PAV outperforms the baseline method in terms of rendering quality under novel head poses, facial expressions, and appearances.

\end{abstract}

==> sec/2_related_backup.tex <==
% Approximately 1.5 columns
\section{Related Work}
\label{sec:related}

% \begin{table}[t]
% \setlength\tabcolsep{8pt} % default: 6pt
% \centering
%      \begin{tabular}{@{} *{5}{l} }
     
%       \footnotesize{\rot{novel view}} &
%       \footnotesize{\rot{novel pose}} &
%       \footnotesize{\rot{generalizable}} &
%       \footnotesize{\rot{relightable}} &
%      \footnotesize{Method} \\
%      \midrule 
%      \OK &        &       &     &   \scriptsize{NeuralBody \cite{peng2021neural}, SelfRecon~\cite{jiang2022selfrecon}   } \\
%      \OK &  \OK   &      &  &  \scriptsize{AnimatableNeRf \cite{peng2021animatable,chen2021animatable}, NeuMan \cite{jiang2022neuman}} \\
%      \OK &  \OK   & \OK  &   & \scriptsize{ANR \cite{raj2020anr}, TNA \cite{shysheya2019textured}, StylePeople \cite{grigorev2021stylepeople}} \\
%      \OK &  &  & \OK     &  \scriptsize{Relighting4D \cite{chen2022relighting}} \\
%      \OK & \OK & \OK & \OK  &  \bf\scriptsize{RANA (Ours)} \\
%      \bottomrule
%      \end{tabular}
%      \caption{Comparison of some of the representative methods for neural human avatar creation. Ours (RANA) is the only method that allows novel view, pose and light synthesis. \vspace{-5mm} 
%      % Furthermore, our method can be trained simultaneously on multiple identities allowing quick fine-tuning for novel subjects.
%      }
% \label{tab:relwork}
% \end{table}

% \noindent\textbf{Neural Head Avatars} 

% \noindent\textbf{Nerf from Photo Collections} 


% \noindent\textbf{Generalizable Nerf} 
% % 1- Overview of genralizable nerf
% % 2- Human body specific generalizable nerf
%     % mentioned about PersonNerf
% % 3- We are the first method addresses learning generalizable head nerf

% \noindent\textbf{Conditional Nerf} 

% \label{sec:relwork_headvatar}
\noindent\textbf{Monocular Neural Head Avatars.}: 





More recent methods learn neural representations of the person from monocular videos and use neural renderers \cite{tewari2020state,tewari2022advances} to directly generate photo-realistic images in the target head pose and facial expression \cite{averbuch2017bringing,siarohin2019first, mallya2022implicit,Zhang_2023_CVPR,kim2018deep,thies2019deferred,Gafni_2021_CVPR,grassal2022neural,zheng2022avatar,athar2022rignerf,zielonka2023instant,chen2023implicit,gao2022reconstructing,bai2023learning}. These methods are generally classified into image-based or 3D-based neural rendering based methods\cite{tewari2020state,tewari2022advances}. The image-based models synthesise the face of a subject without relying on any representation of 3D space. Existing image-based approaches either employ learned warping fields \cite{averbuch2017bringing,siarohin2019first} to deform an input image or encoder-decoder architecture where decoder synthesize the output image \cite{mallya2022implicit,nirkin2019fsgan,wang2018high,zakharov2020fast}. Even though these methods produce high-quality results, they suffer from artifacts for strong head pose and expression changes due to the lack of 3D geometry. The 3D-based neural rendering methods, on the other hand, relied on 3D Morphable Models (3DMM) \cite{egger20203d}. These methods are generally classified into explicit and implicit models. Explicit models utilize 2D neural rendering methods \cite{tewari2020state,tewari2022advances} and rely on neural networks which can be conditioned on coarse RGB renderings based on a linear texture model \cite{kim2018deep}, uv-maps \cite{buhler2021varitex} or latent feature maps \cite{thies2019deferred}. Although these techniques produce high-quality renderings, they are confined to operating within a 2D image space and are limited to craniofacial structures. To tackle this, implicit neural representations for modeling 3D faces have recently become a major focus of attention. In particular, NeRFs \cite{mildenhall2021nerf} shows photorealistic face image synthesis in novel poses and expressions \cite{Gafni_2021_CVPR, grassal2022neural, zheng2022avatar, athar2022rignerf, zielonka2023instant}.

[To Be Continued]

% Mention about their differences like implicit or explicit deformation field. 

% However, NeRFs require per-identity optimization, maintaining the consistent appearance of the same subject. The recent method \cite{wang2022morf} is the only exception; however, they require multiview images recorded in a controlled environment. 

% Our method falls into the implicit 3D neural rendering paradigm as we build our system on top of dynamic head NeRF. In particular, we take inspiration from Insta \cite{zielonka2023instant} for designing our framework. 

% Among implicit models, ours is the only method that allows learning dynamic head nerf model from unstructured video collection. 


 
% Image-based and 3D geomeetry-based head avatars
% Implicit and Explicit Methods (look at grassal2022neural)
% Multiview captures of static and dynamic heads (zielonka2023instant,)
% Learning head avatars from monocular video
% Rigged Neural Radiance field for head avatars, but they are trained using one appearance of one subject. 
% Implicit methods -> implicit (grassal2022neural) and explicit (zielonka2023instant) modeling of deformation. Explicit deformation modeling introduces fine grained control
%However, these methods are only limited to single appearance of a single identity. Our method is the first approach bla bla. (LA RANA)
% Implicit methods -> Since the training time for implicit models (), fast training approaches are applied to train neural head avatars (). In this paper we are using multi-resolution hash encoding for faster training time. 

% Previous works focused on a single identity and a single appearance of that identity and captured long sequences of videos. 
% Multi-identity Nerf -> is the first work but requires multiview capture setup. 

%MoRF \cite{wang2022morf} method learns identity-specific code vectors for density and radiance fields for head nerf. However, the proposed method requires multi-view captures. 

\noindent\textbf{Neural Radiance Fields from Data Collections}
\label{sec:relwork_nerf_data_collect}

[To Be Continued]

% Nerf in the wild
% Morf -> 
% PersonNerf -> for human body and from photos
% For the deformable dynamic head avatar, this problem is not visited. 

% YOTO -> for human body

%\noindent\textbf{Neural Rendering from Unstructured Photo Collections.} 
%\bk{joint camera and RF modeling papers?}

%\noindent\textbf{Controllable and Editable NeRF.} 
%\bk{restrict only to head animation?}
% "Editing Conditional Radiance Fields"

\input{figures/fig_overview.tex}

